VISTA: Triplet-Supervised Video Style Transfer with Diffusion Transformers

Video style transfer aims to render videos in a target artistic style while preserving content, structure, and motion. While image stylization has advanced rapidly, video stylization remains challenging due to temporal inconsistency. Most existing methods stylize frames or keyframes and enforce consistency via heuristic temporal propagation, which is brittle under occlusions, disocclusions, and long-term motion, leading to drift and flickering artifacts. We argue that a fundamental bottleneck lies in the lack of large-scale triplet data and a principled training paradigm that jointly models and disentangles style, content, and motion.To address this, we introduce VISTA-1000, a synthetic dataset with 1,000 styles and motion-aligned triplets of style reference, clean video, and stylized video, and propose a diffusion-transformer-based in-context video style transfer framework with a lightweight style adapter for robust style extraction. Extensive experiments demonstrate SOTA performance in style fidelity, temporal consistency, and content preservation.

==> sec/0_abstract.tex <==

% 视频风格迁移旨在在保持内容、结构与运动的同时，将视频渲染为目标艺术风格。尽管图像风格化进展迅速，视频风格化仍受时间一致性问题所限制。现有方法多对单帧或关键帧进行风格化，并通过启发式时序传播（如基于光流的对齐与warp）维持一致性，但该过程在遮挡、新显露区域与长时序运动下易失效，产生风格漂移与闪烁伪影。我们认为其根本瓶颈在于缺乏能够联合建模并解耦风格、内容与运动的大规模三元组数据，以及与之配套的原则性训练范式与模型设计。为此，我们提出 VISTA-1000：一个包含 1,000 种风格的合成数据集，提供运动对齐的三元组——风格参考图、干净视频与风格化视频。基于 VISTA-1000，我们提出一种基于扩散 Transformer 的上下文学习视频风格迁移框架，并引入轻量级风格适配器以实现鲁棒的风格提取。大量实验表明，我们的方法在风格保真度、时间一致性与内容保持方面达到当前最先进水平。

\begin{abstract}
Video style transfer aims to render videos in a target artistic style while preserving content, structure, and motion. While image stylization has advanced rapidly, video stylization remains challenging due to temporal inconsistency. Most existing methods stylize frames or keyframes and enforce consistency via heuristic temporal propagation, which is brittle under occlusions, disocclusions, and long-term motion, leading to drift and flickering artifacts. We argue that a fundamental bottleneck lies in the lack of large-scale triplet data and a principled training paradigm that jointly models and disentangles style, content, and motion.To address this, we introduce VISTA-1000, a synthetic dataset with 1,000 styles and motion-aligned triplets of style reference, clean video, and stylized video, and propose a diffusion-transformer-based in-context video style transfer framework with a lightweight style adapter for robust style extraction. Extensive experiments demonstrate SOTA performance in style fidelity, temporal consistency, and content preservation.

\end{abstract}

% 如何验证 clean 与 stylized 在结构与 motion 上严格对齐？给定量指标。
% 视频风格迁移本质规律（如时空纠缠、非线性风格映射）
% 合成数据与现实世界的“鸿沟”
% 图像数据怎么用， OC


==> sec/1_intro-old.tex <==
% \section{Introduction}
% \label{sec:intro}
% Video style transfer aims to generate a stylized version of a video that inherits the artistic appearance of a given reference while faithfully preserving the original content, structure, and motion.
% It represents one of the most challenging problems in controllable video generation, as the model must simultaneously maintain temporal coherence, geometric stability, and consistent texture propagation across frames.
% In other words, an ideal stylized video should not only capture the target artistic style but also exhibit smooth temporal transitions and stable visual quality over time.

% Existing video stylization approaches often rely on handcrafted heuristics or training-free techniques to maintain temporal consistency.
% Typical strategies propagate features or colors across frames using optical flow, align content and style through AdaIN normalization, or incorporate auxiliary signals such as depth or edge maps to preserve structure.
% While these methods can produce visually pleasing short sequences, their performance quickly degrades as motion accumulates, leading to information loss and temporal artifacts.
% Moreover, intermediate or compressed representations tend to discard fine-grained spatial details, resulting in style fading, structural distortion, and flickering.
% Fundamentally, such heuristic pipelines depend more on engineered constraints than on learned knowledge, which limits their capacity for long-term temporal stability.

% To overcome these limitations, we propose a data-driven and end-to-end framework for video style transfer built upon the large-scale pretrained Diffusion Transformer (WAN 2.2).
% Unlike previous methods that impose handcrafted temporal constraints, our framework learns both style and motion consistency directly from data through In-Context Learning.
% Specifically, we construct a high-quality synthetic triplet dataset, where each sample consists of a style reference image, a stylized video, and its corresponding clean video.
% In each triplet, the style reference and the stylized video share the same artistic domain but originate from different sources, while the stylized and clean videos share identical content, layout, and motion but differ in appearance.
% This design prevents content leakage and allows the model to learn the intrinsic mapping between artistic style and temporal dynamics.

% During training, the clean video is concatenated as the conditional sequence, and the stylized video serves as the denoising target within the diffusion process.
% This in-context formulation enables the model to preserve fine content details while achieving consistent frame-to-frame stylization—without relying on optical flow or depth supervision.
% To further enhance style fidelity, we introduce a lightweight Style Adapter that encodes the reference image into fine-grained style embeddings and injects them into the transformer’s attention layers.
% The adapter provides precise and temporally stable style control while maintaining structural coherence.
% Trained entirely on our synthetic triplet data, the resulting model achieves superior style fidelity, temporal smoothness, and overall visual quality compared to existing training-free and propagation-based methods.

% Extensive experiments demonstrate that our approach achieves state-of-the-art temporal consistency and style realism.
% The results confirm a simple yet fundamental insight:
% True consistency in video stylization arises from data-driven learning rather than handcrafted propagation.

% \begin{itemize}
%     \item \textbf{Data-driven video-to-video stylization framework.} 
%     Data-driven framework for video-to-video stylization.
% We propose an end-to-end diffusion transformer framework that achieves high-quality, temporally coherent video stylization with consistent style, content, and motion.
    
%     \item \textbf{In-context learning and style adapter for consistency and control.}
% We employ in-context learning to enforce temporal coherence and introduce a lightweight Style Adapter for precise style injection and stable stylization.
    
%     \item \textbf{Large-scale triplet dataset for video stylization.} 
%     We construct a high-quality synthetic triplet dataset containing style references, stylized videos, and clean counterparts, and conduct extensive experiments validating the effectiveness of our approach.
% \end{itemize}

% \section{Introduction}

% Video style transfer aims to transform an input video into a target artistic style while preserving its original content, structure, and motion.
% While significant progress has been achieved in image-level stylization, extending these methods to videos remains fundamentally challenging due to stringent temporal consistency requirements and severe data limitations.
% In practice, an effective video style transfer system must maintain coherent appearance across frames, preserve motion dynamics, and faithfully apply the target style without introducing flickering or structural distortion.

% From a first-principles perspective, successful video style transfer requires a specific form of supervision that is largely absent in existing datasets.
% Ideally, training data should consist of triplets:
% (1) a \emph{style reference image} that shares the same artistic style but depicts different content,
% (2) a \emph{clean input video} representing the original content and motion, and
% (3) a \emph{stylized output video} that preserves the input video’s motion and structure while adopting the target style.
% Such triplets explicitly disentangle style, content, and motion, enabling a model to learn how to transfer appearance while maintaining temporal coherence.

% However, existing public video stylization benchmarks fall far short of this requirement.
% Most datasets contain only a handful of styles—often fewer than five—and typically provide neither paired pre-/post-stylization videos nor corresponding style reference images.
% In many cases, style information is implicit, unpaired, or entirely absent.
% As a result, current methods are forced to rely on image-level style encoders trained on unrelated image datasets, combined with heuristic temporal propagation mechanisms such as optical flow or frame-wise regularization.
% While these techniques can mitigate flickering in short clips, they fundamentally fail to learn style–motion alignment and break down under long-term or complex motion.

% To address this core limitation, we adopt a data-centric approach grounded in first principles.
% We introduce \textbf{VISTA-1000}, a large-scale video style transfer dataset explicitly designed to provide the missing supervision.
% VISTA-1000 contains \textbf{1,000 distinct artistic styles}, each associated with \textbf{four pairs of semantically different but stylistically consistent videos}.
% For every video, we construct both a stylized version and its corresponding de-stylized (clean) counterpart, forming paired input–output videos.
% Importantly, keyframes from one video naturally serve as style reference images for the other videos within the same style group, yielding rich triplets of \emph{(style reference image, clean input video, stylized output video)}.
% This structure tightly couples style and content while preserving motion alignment, providing an ideal foundation for learning video style transfer.

% Built upon this dataset, we propose a data-driven video style transfer framework based on \emph{in-context learning} with diffusion transformers.
% By concatenating conditional video tokens and denoising video tokens within a shared context, the model learns motion-aligned style transfer directly from paired video supervision.
% To further enhance style extraction from a single reference image, we introduce a lightweight \emph{Style Adapter}, pretrained on large-scale image data and post-trained on style images, which injects fine-grained style information into the model via cross-attention.
% Together, these components enable robust, temporally consistent video stylization without relying on handcrafted temporal heuristics.

% Extensive experiments demonstrate that our approach achieves state-of-the-art performance in style fidelity, temporal consistency, and content preservation across diverse styles and motion patterns.
% Our results highlight a central insight: the primary bottleneck of video style transfer is not model capacity, but the lack of properly structured data, and addressing this bottleneck unlocks substantial performance gains.

% In summary, our contributions are threefold.

% \begin{itemize}
%     \item We introduce VISTA-1000, a large-scale video style transfer dataset constructed from first principles, containing 1,000 styles with paired clean and stylized videos and naturally formed triplets of style reference images, input videos, and output videos, explicitly disentangling style, content, and motion.
    
%     \item We propose a data-driven video style transfer framework that combines \emph{in-context learning} with a lightweight \emph{Style Adapter}, enabling temporally consistent and style-faithful video stylization without optical flow or handcrafted temporal constraints.
    
%     \item Third, through extensive quantitative and qualitative evaluations, we demonstrate that our method significantly outperforms existing image-based and heuristic video stylization approaches, establishing new state-of-the-art results in style consistency, temporal stability, and content preservation.
% \end{itemize}

\section{Introduction}

Video style transfer aims to transform an input video into a target artistic style while preserving its original content, structure, and motion.
Although image stylization has progressed rapidly, extending it to videos remains challenging because temporal coherence must be maintained over long sequences under complex motion.
An effective video stylization system should produce consistent appearance across frames, preserve motion dynamics, and avoid flickering artifacts or structural distortions.

Most existing approaches follow a two-stage paradigm: they stylize frames (or a few keyframes) using image-based style representations, and then enforce temporal consistency via heuristic propagation mechanisms such as optical-flow warping, feature propagation, or frame-wise regularization.
While these strategies can reduce short-term flicker, they are inherently fragile under occlusions, disocclusions, and non-rigid motion.
In particular, imperfect alignment introduces errors that accumulate over time, leading to drift, texture swimming, and unstable stylization in long videos.
These failure modes suggest that temporal consistency cannot be reliably achieved by post-hoc propagation alone.

From a machine learning perspective, we argue that the above limitations stem from a more fundamental issue: current training setups lack both properly structured supervision and a principled learning paradigm that jointly models and disentangles \emph{style}, \emph{content}, and \emph{motion}.
Ideally, a model should be trained with triplets consisting of
(1) a \emph{style reference image} that provides appearance cues,
(2) a \emph{clean input video} that specifies content and motion, and
(3) a \emph{stylized output video} that preserves the input motion and structure while adopting the target style.
Such triplets explicitly separate appearance from motion dynamics, enabling the model to learn motion-aligned style transfer rather than relying on fragile temporal heuristics.
However, existing public video stylization benchmarks provide only a handful of styles and rarely contain paired clean/stylized videos or explicit style references, making it difficult to learn this disentanglement in a data-driven manner.

To address this bottleneck, we propose a data-centric and method-centric solution that couples structured supervision with a dedicated training framework.
We introduce \textbf{VISTA-1000}, a large-scale synthetic dataset designed from first principles for learning video style transfer.
VISTA-1000 contains \textbf{1,000 distinct artistic styles}, and for each style, it provides \textbf{four pairs of semantically different but stylistically consistent videos}.
For every video, we construct both a stylized version and its corresponding de-stylized (clean) counterpart, yielding paired input--output videos.
Moreover, keyframes from one video naturally serve as style reference images for other videos within the same style group, forming abundant triplets of \emph{(style reference image, clean input video, stylized output video)}.
This design enables large-scale training with explicit supervision that disentangles style, content, and motion.

Built upon VISTA-1000, we propose a diffusion-transformer-based video style transfer framework that learns style--motion alignment directly from paired video supervision.
Our key idea is to perform \emph{in-context learning} for conditional video generation: we concatenate conditional video tokens (from the clean input) with denoising video tokens (for the stylized output) within a shared context, allowing the model to learn motion-aligned appearance transfer through joint attention.
To robustly extract style from a single reference image, we further introduce a lightweight \emph{Style Adapter} that injects fine-grained style information via cross-attention.
The adapter is pretrained on large-scale image data and post-trained on style images, making it both effective and efficient.
Together, these components enable temporally consistent video stylization without optical flow or handcrafted temporal constraints.

Extensive experiments demonstrate that our approach achieves state-of-the-art performance in style fidelity, temporal consistency, and content preservation across diverse styles and motion patterns.
Beyond improved results, our study reveals a central insight: scaling video style transfer requires not only larger datasets, but also structured supervision and a learning paradigm that can exploit it effectively.

In summary, our contributions are threefold:
\begin{itemize}
    \item We revisit video style transfer from a learning perspective and highlight the importance of structured triplet supervision that connects \emph{style reference images}, \emph{clean input videos}, and \emph{stylized output videos} for learning temporally coherent stylization.
    
    \item We introduce \textbf{VISTA-1000}, a curated triplet dataset with 1,000 artistic styles, where each style provides paired clean/stylized videos and naturally formed triplets for disentangling style, content, and motion.
    
    \item We propose a diffusion-transformer-based video style transfer framework with in-context conditioning and a lightweight \emph{Style Adapter}, and demonstrate competitive performance in style fidelity, temporal consistency, and content preservation on diverse styles and motion patterns.
\end{itemize}


